Randomized Kaczmarz for Rank Aggregation from Pairwise Comparisons

We revisit the problem of inferring the overall ranking among entities in the framework of Bradley-Terry-Luce (BTL) model, based on available empirical data on pairwise preferences. By a simple transformation, we can cast the problem as that of solving a noisy linear system, for which a ready algorithm is available in the form of the randomized Kaczmarz method. This scheme is provably convergent, has excellent empirical performance, and is amenable to on-line, distributed and asynchronous variants. Convergence, convergence rate, and error analysis of the proposed algorithm are presented and several numerical experiments are conducted whose results validate our theoretical findings.

==> RealData.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\subsection{Real Data}
We wanted to see the performance of this algorithm on real data with some head to head statistics where all players have not played each other. Professional Lawn Tennis seemed to be a good option. We have scraped the data of all the head to head matches of $154$ players as available on November, 2015. We have a connectivity of 0.54 in the observed data with an average $2.5$ comparison per edge. A regularization was necessary to use this algorithm for real data as all wins for $i$ over $j$ would yield us $y_{ij} = \infty$ and $y_{ji} = -\infty$ for which we would not be able to iterate. Hence we need to redefine the equation for $\hat{p}_{ij}$ as: 
$$\hat{p}_{ij} = \frac{\sum X_{ij} + \epsilon}{\sum X_{ij} +\sum X_{ji} + 2\cdot \epsilon}$$
Using value of $\epsilon = 1$, we get Table \ref{table:tennis}. We can see that just by using the winning ratio, Rafael Nadal would have been ranked first but using the fact of the opponent's rating, Roger Federer grabs the top position. Also since we have taken all the matches into account, the people who have performed well in the past but not doing so good currently like Jarkko Nieminen and Jurgen Melzer are ranked much higher then their current rankings.

\begin{table}[t]
\centering
\caption{Rank Aggregation for Tennis Players based on Pairwise Comparisons}
\label{table:tennis}
\begin{tabular}{@{}cccccc@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ATP\\ Rank\end{tabular}} & \multirow{2}{*}{Name} & \multirow{2}{*}{Degree} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Win\\ Ratio\end{tabular}} & \multicolumn{2}{c}{$\epsilon$ = 1}                           \\ \cmidrule(l){5-6} 
                                                                    &                       &                         &                            & \multicolumn{1}{l}{Rank} & \multicolumn{1}{l}{$w_i$} \\ \midrule
1                                                                   & Novak Djokovic        & 88                      & 4.37                       & 2                        & 2.18                   \\
2                                                                   & Andy Murray           & 94                      & 3.03                       & 4                        & 1.79                   \\
3                                                                   & Roger Federer         & 88                      & 4.51                       & 1                        & 2.30                   \\
4                                                                   & Stan Wawrinka         & 96                      & 1.64                       & 9                        & 1.18                   \\
5                                                                   & Rafael Nadal          & 96                      & 4.73                       & 3                        & 1.99                   \\
6                                                                   & Tomas Berdych         & 97                      & 1.71                       & 6                        & 1.30                   \\
$\vdots$                                                                    &   $\vdots$                    & $\vdots$ & $\vdots$ & $\vdots$                          & $\vdots$                          \\
150                                                                 & Blaz Kavcic           & 103                      & 0.88                       & 85                       & 0.56                   \\
151                                                                 & Karen Khachanov       & 28                     & 0.35                       & 152                      & 0.36                   \\
152                                                                 & Jarkko Nieminen       & 100                     & 0.81                       & 46                       & 0.66                   \\
153                                                                 & Jurgen Melzer         & 102                      & 0.99                       & 29                       & 0.74                   \\
154                                                                 & Jordan Thompson       & 26                   & 0.35                       & 153                      & 0.35                   \\
\multicolumn{1}{l}{}                                                & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}     \\ \bottomrule
\end{tabular}
\end{table}
